Seamlessly Integrating Factual Information and Social Content with Persuasive Dialogue

Complex conversation settings such as persuasion involve communicating changes in attitude or behavior, so users' perspectives need to be addressed, even when not directly related to the topic. In this work, we contribute a novel modular dialogue system framework that seamlessly integrates factual information and social content into persuasive dialogue. Our framework is generalizable to any dialogue tasks that have mixed social and task contents. We conducted a study that compared user evaluations of our framework versus a baseline end-to-end generation model. We found our framework was evaluated more favorably in all dimensions including competence and friendliness, compared to the end-to-end model which does not explicitly handle social content or factual questions.

==> tables/persuasion_examples.tex <==
\begin{table*}[]
\small
\centering
\begin{tabular}{|l|l|}
\hline
\textbf{Dialogue Act/Persuasive Strategy} & \textbf{Example Utterance} \\ \hline
Greeting & Hello there! How are you doing? \\ \hline
Source-related inquiry & Have you heard of the organization Save the Children? \\ \hline
% Task-related inquiry & Have you donated to a charity before? \\ \hline
Personal-related inquiry & Do you have kids yourself? \\ \hline
Credibility appeal & \begin{tabular}[c]{@{}l@{}}Save the Children is an international non-governmental organization that \\ promotes children's rights, provides relief, and helps support children in \\ developing countries.\end{tabular} \\ \hline
Emotional appeal & \begin{tabular}[c]{@{}l@{}}It make me feel sad to see that so many children are suffering from \\ poverty and hunger.\end{tabular} \\ \hline
Logical appeal & \begin{tabular}[c]{@{}l@{}}Donations are extremely important in order for children to have their \\ rights to healthcare, education, safety, etc. If you were to donate, you \\ would be making a huge impact on these children and on the world.\end{tabular} \\ \hline
Self-modeling & I think I'll donate a bit of my money to Save the Children, \$2. \\ \hline
Foot-in-the-door & Every little bit helps. Even a small amount! \\ \hline
Personal story & \begin{tabular}[c]{@{}l@{}}Someone told me that he and his brother replaced birthday gifts \\ with charity donations a few years ago, and it was a really rewarding \\ experience for them.\end{tabular} \\ \hline
Propose donation & Would you like to make a donation to Save the Children? \\ \hline
Closing & Thank you, it's been lovely talking to you. Enjoy your day and bye! \\ \hline
\end{tabular}
\caption{Examples of each dialogue act from \persuasion used for the chatbot.}
\label{dialogue_acts}
\end{table*}

==> tables/results.tex <==

\begin{table*}[t]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{The chatbot...}                                        & \textbf{Baseline ($\mu\pm\sigma$)} & \textbf{RAP ($\mu\pm\sigma$)} & \textbf{Invoked Social} & \textbf{Invoked Factual} \\ \hline
is competent                                                   & 2.53$\pm$0.82                          & 3.00$\pm$1.06**   & 2.98$\pm$1.08**                          & \textbf{3.03$\pm$1.00**}                     \\ \hline
is natural                                                     & 2.35$\pm$1.03                          & \textbf{2.65$\pm$1.00}  & 2.65$\pm$1.04                          & 2.58$\pm$0.85                        \\ \hline
increased my intention to donate                               & 3.00$\pm$1.17                           & 3.19$\pm$1.13    & 3.16$\pm$1.14                          & \textbf{3.33$\pm$1.06}                    \\ \hline
is persuasive                                                  & 2.63$\pm$1.05                           & \textbf{2.72$\pm$1.10}  & 2.65$\pm$1.12                          & 2.70$\pm$1.00                      \\ \hline
is well-intentioned                                            & 3.65$\pm$1.01                           & 3.84$\pm$1.01   & 3.86$\pm$1.03                          & \textbf{3.97$\pm$0.94}                     \\ \hline
is friendly                                                    & 3.16$\pm$1.05                           & 3.39$\pm$1.12   & 3.41$\pm$1.10                          & \textbf{3.58$\pm$1.12*}                     \\ \hline
is intelligent                                                 & 2.51$\pm$0.92                           & 2.74$\pm$1.07   & 2.73$\pm$1.09                          & \textbf{2.79$\pm$1.07}                    \\ \hline
is convincing                                                  & 3.02$\pm$1.08                           & 3.11$\pm$0.89   & 3.10$\pm$0.89                          & \textbf{3.15$\pm$0.89}                     \\ \hline
is confident                                                   & 3.35$\pm$1.01                           & 3.72$\pm$0.89** & 3.71$\pm$0.91*                          & \textbf{3.76$\pm$0.78*}                        \\ \hline
is a strong reason for donating                 & 2.67$\pm$0.92                           & \textbf{2.84$\pm$1.02}   & 2.78$\pm$1.03                          & 2.82$\pm$1.09                     \\ \hline
was dishonest                                                  & 2.14$\pm$0.89                           & 1.91$\pm$0.80   & 1.94$\pm$0.83                          & \textbf{1.88$\pm$0.77}                     \\ \hline
% put thoughts in my mind about wanting to donate to the charity & 0,0                           & 0,0                       \\ \hline
% is something I agree with overall                              & 0,0                           & 0,0                       \\ \hline
% tried to pressure me                                           & 0,0                           & 0,0                       \\ \hline
\end{tabular}
\caption{Comparing mean and standard deviation of the baseline (BART) and \framework from the post-task survey. Statistically significant differences compared to the baseline at $\alpha=0.05$ are denoted with **; significant differences at $\alpha=0.1$ are denoted with *. 51 participants used the baseline and 57 participants used \framework. Of the 57 \framework participants, 51 had conversations that triggered the Social Response Module and 33 conversations triggered the Factual Answer Module. 24 conversations triggered the Social Response Module but not the Factual Answer Module, and 6 conversations triggered the Factual Answer Module but not the Social Response Module.}
\label{evaluation}
\end{table*}
